Can We Theoretically Quantify the Impacts of Local Updates on the Generalization Performance of Federated Learning?

Federated Learning (FL) has gained significant popularity due to its effectiveness in training machine learning models across diverse sites without requiring direct data sharing. While various algorithms along with their optimization analyses have shown that FL with local updates is a communication-efficient distributed learning framework, the generalization performance of FL with local updates has received comparatively less attention. This lack of investigation can be attributed to the complex interplay between data heterogeneity and infrequent communication due to the local updates within the FL framework. This motivates us to investigate a fundamental question in FL: Can we quantify the impact of data heterogeneity and local updates on the generalization performance for FL as the learning process evolves? To this end, we conduct a comprehensive theoretical study of FL's generalization performance using a linear model as the first step, where the data heterogeneity is considered for both the stationary and online/non-stationary cases. By providing closed-form expressions of the model error, we rigorously quantify the impact of the number of the local updates (denoted as $K$) under three settings ($K=1$, $K<\infty$, and $K=\infty$) and show how the generalization performance evolves with the number of rounds $t$. Our investigation also provides a comprehensive understanding of how different configurations (including the number of model parameters $p$ and the number of training samples $n$) contribute to the overall generalization performance, thus shedding new insights (such as benign overfitting) for implementing FL over networks.

==> RelatedWork.tex <==


\section{Related Work} \label{sec:relatedWork}

\textbf{1) Generalization performance of FL.}
In the literature, there has been relatively limited studies on the generalization of FL. 
We categorize these works into two distinct classes.
The first line of works employs the traditional analytical tools from statistical learning.
%
\citet{yuan2022what} assumes that clients’ data distributions are drawn from a meta-population distribution. Accordingly, they define two generalization gaps in FL: one is the participation generalization gap to measure the difference between the empirical and expected risk for participating clients, the same as the definition in classic statistical learning; the second is the non-participation generalization gap, which measures the difference of the expected risk between participating and non-participating clients.
Following this two-level distribution framework, sharper bounds are provided ~\cite{hu2023generalization}.
% as $\mathcal{O}(\frac{1}{Mn})$ for participation gap and $\mathcal{O}(\frac{1}{M})$ for non-participation gap, respectively~\cite{hu2023generalization}.
\citet{zhao2023federated} utilized the Probably Approximately Correct (PAC) Bayesian framework to investigate a tailored generalization bound for heterogeneous data in FL.
More works utilize similar tools to study the generalization in FL~\citep{chor2023more,barnes2022improved,sefidgaran2022rate,sun2023understanding,sefidgaran2023federated,huang2021fl}.
%

The second class of works studied the training dynamic near a manifold of minima and the effect of stochastic gradient noise on generalization. They used ``sharpness'' as a useful tool for generalization. \citet{caldarola2022improving} and \citet{shi2023make} investigated the generalization behavior through the lens of the geometry of the loss and Hessian eigenspectrum, linking the model’s lack of generalization capacity to the sharpness of the solution under ideal client participation.
Based on the sharpness, ~\citet{qu2022generalized} proposed a momentum algorithm with better generalization.
%
In addition, \citet{gu2022and} utilizes the stochastic differential equation (SDE) approximation to study the long-term behavior of the learning process.
They showed that utilizing local steps always exhibits better generalization under appropriate conditions, including a sufficiently small learning rate, enough number of communication rounds, and the local steps being tuned.
%
All of these existing studies primarily yield asymptotic results by focusing on domain changes or describing limiting behavior such as sufficiently large communication rounds and fine-tuned local steps. 
Consequently, they do not establish a direct, quantifiable relationship that demonstrates how key factors—namely, data heterogeneity, the local update process, and the communication round—affect the generalization performance of FL.
% So, they do not provide an explicit relationship to show how these critical factors, such as the local update process, the number of communication rounds, and data heterogeneity affect the generalization of FL in general. 
In this paper, we achieve the explicit quantification of the impact of data heterogeneity, local update steps, and the total number of communication rounds on the generalization performance within the context of a federated linear regression model.

\textbf{2) Model Averaging.}
Model averaging, as discussed in works such as~\citep{dobriban2021distributed, kamp2019efficient, kamp2014communication}, shares a resemblance to federated learning due to the commonality of employing a periodic averaging process. However, a fundamental distinction lies in the problem setting: federated learning assumes different local data distributions for each client, while model averaging assumes that the data in each client is sampled from one identical distribution. In this context, it's noteworthy that our results can be regarded as a degeneration to their setting under the assumption of independently and identically distributed (IID) data.
